Hamiltonian dynamics simulation using linear combination of unitaries on an ion trap quantum computer

The linear combination of unitaries (LCU) method has proven to scale better than existing product formulas in simulating long time Hamiltonian dynamics. However, given the number of multi-control gate operations in the standard prepare-select-unprepare architecture of LCU, it is still resource-intensive to implement on the current quantum computers. In this work, we demonstrate LCU implementations on an ion trap quantum computer for calculating squared overlaps $|\langle \psi(t=0)|\psi(t>0)\rangle|^2$ of time-evolved states. This is achieved by an optimized LCU method, based on pre-selecting relevant unitaries, coupled with a compilation strategy which makes use of quantum multiplexor gates, leading to a significant reduction in the depth and number of two-qubit gates in circuits. For $L$ Pauli strings in a Taylor series expanded $n$-qubit-mapped time evolution operator, we find a two-qubit gate count of $2^{\lceil log_2(L)\rceil}(2n+1)-n-2$. We test this approach by simulating a Rabi-Hubbard Hamiltonian.

==> sections/Method/oaa.tex <==
\subsection{Oblivious amplitude amplification}

To boost the LCU success probability in Eq.~\ref{eq:lcu_success_prob}, we apply the amplification operator $A = -WRW^\dagger R $, where $W$ is the LCU operator acting on both the ancilla and system registers, and $R = (I - 2|\bar{0}\rangle\langle\bar{0}|) \otimes I$ is the reflection operator. After a single application of $A$, the expected probability becomes\footnote{This is exact if $\Upsilon$ is unitary. Otherwise, a slight modification has to be done. Derivation of Eq.~(\ref{eq:p_amp}) is shown in Appendix~\ref{appendix:oaa}. }
\begin{align}
\label{eq:p_amp}
    p_{amp} = p (4p-3)^2.
\end{align}
This implies that if $p\ll 0.5$, then after one round of amplification, the success probability should be improved by about a factor of $9$. The general case for a single application of $\langle\psi|\Upsilon^\dagger \Upsilon|\psi\rangle \not\approx 1$, the amplified probability is
\begin{widetext}
\begin{align}
\label{eq:p_amp_gen}
    p_{amp} =\frac{1}{|\alpha|_1^2} \left\langle \psi \left| \left( 3\Upsilon - \frac{4}{|\alpha|_1^2}\Upsilon \Upsilon^\dagger \Upsilon \right)^\dagger \left( 3\Upsilon - \frac{4}{|\alpha|_1^2}\Upsilon \Upsilon^\dagger \Upsilon \right) \right|\psi \right\rangle.
\end{align}
\end{widetext}
As the LCU alone is already an expensive algorithm, the circuit depth triples for every application of $A$. 


==> sections/Results/hubbard.tex <==
\subsection{Hubbard model}

==> sections/Results/molecular.tex <==
\subsection{Quantum chemistry Hamiltonian}



==> sections/changes.tex <==
\clearpage
\section{Summary of changes}

\begin{enumerate}
  \item Abstract
  
  \item $dt$ to $\tau$ and a few notations in the background section.

  
  \item Yuta on Eq.(2): Can you calculate how many terms are needed to achieve an error epsilon, and compare it with the truncated Taylor?In the original Berry's paper, they used K-queries to the controlled-H in the SELECT part of the LCU, which allows them achieving \tilde{O}(t) scaling. However, if you naively implement LCU of Eq(2) above, I expect $O(t^2/\epsilon)$$ scaling.

M: This would be a good but difficult exercise. 
In practice though, we set a cutoff to the terms based on the magnitude of $\alpha_j$, and the number of terms (400-500) didn't vary wildly as a function of time, while the precision varies non-monotonically between $10^{-7.3}$ and $10^{-6}$. (And in the end, these 500 terms are further reduced given some conditions which is the main thesis of the paper.)

Also, $O(t^2/\epsilon)$ seems a bit naïve as well, since we know that the number of terms is bounded by $4^s$, where s is the system size.

\item In background section, removed "Performing OAA triples the circuit depth but improves the success probability by a factor of $9$." from the last paragraph.

\item Discussion section
Yuta on 2nd paragraph 2nd sentence: How should we reconcile this from the viewpoint of no-fast forwarding?
Michelle: Edited 2nd paragraph

\item Addition of Supporting figures section in Appendix

\end{enumerate}

==> sections/results.tex <==
\section{Results}

To demonstrate Hamiltonian dynamics simulations, we start with the simplest light-matter interaction in the form of the Jaynes-Cummings system. We show the quantitative results in Appendix~\ref{appendix:jc} where we calculate the transition probability of $4$-qubit states as a function of time. We consider both LCU and LCU with OAA methods, without the LCU reduction technique described in Sec.~\ref{sec:sq_overlap}, and compare these with the naïve Trotter approach. These simulations are performed on Quantinuum's emulator H1-1E without the noise model. The LCU, without OAA, circuits use $10$ qubits and have an average depth of $1280$ and $714$ \CX gates. Upon employing the preselection technique in Sec.~\ref{sec:sq_overlap}, the number of LCU terms is reduced to $2$, requiring only $1$ ancillary qubit. This is a good illustration of the effectivity of Sec.~\ref{sec:sq_overlap}, but may be inconsequential for testing the LCU algorithm on a hardware. 
\input{sections/Results/rh}
